OmniSeg3D: Omniversal 3D Segmentation via Hierarchical Contrastive Learning

Towards holistic understanding of 3D scenes, a general 3D segmentation method is needed that can segment diverse objects without restrictions on object quantity or categories, while also reflecting the inherent hierarchical structure. To achieve this, we propose OmniSeg3D, an omniversal segmentation method aims for segmenting anything in 3D all at once. The key insight is to lift multi-view inconsistent 2D segmentations into a consistent 3D feature field through a hierarchical contrastive learning framework, which is accomplished by two steps. Firstly, we design a novel hierarchical representation based on category-agnostic 2D segmentations to model the multi-level relationship among pixels. Secondly, image features rendered from the 3D feature field are clustered at different levels, which can be further drawn closer or pushed apart according to the hierarchical relationship between different levels. In tackling the challenges posed by inconsistent 2D segmentations, this framework yields a global consistent 3D feature field, which further enables hierarchical segmentation, multi-object selection, and global discretization. Extensive experiments demonstrate the effectiveness of our method on high-quality 3D segmentation and accurate hierarchical structure understanding. A graphical user interface further facilitates flexible interaction for omniversal 3D segmentation.

==> sec/0_abstract.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}
   % General 3D segmentation is crucial for achieving holistic understanding of anything in the 3D space.  
   Towards holistic understanding of 3D scenes, a general 3D segmentation method is needed that can segment diverse objects without restrictions on object quantity or categories, while also reflecting the inherent hierarchical structure.
   %
   To achieve this, we propose OmniSeg3D, an omniversal segmentation method aims for segmenting anything in 3D all at once. 
   %
   The key insight is to lift multi-view inconsistent 2D segmentations into a consistent 3D feature field through a hierarchical contrastive learning framework, which is accomplished by two steps. 
   %, simultaneously distilling the underlying hierarchical structure.
   %
   % This is accomplished \haiyang{by clustering image features rendered from the 3D feature field hierarchically at different levels of segmentation blocks, and contrasting them otherwise}. Additionally, a novel hierarchical representation based on any category-agnostic 2D segmentations is implemented to guide the training order of feature clustering.
   %
   Firstly, we design a novel hierarchical representation based on category-agnostic 2D segmentations to model the multi-level relationship among pixels. 
   Secondly, image features rendered from the 3D feature field \jinzhi{are} clustered at different levels of 2D segmentation blocks, which \jinzhi{can be} further drawn closer or \yixuan{pushed} apart according to the hierarchical relationship between different levels.
   %
   \yixuan{In tackling} the challenges posed by inconsistent 2D segmentations, this framework yields a global consistent 3D feature field, which further enables hierarchical segmentation, multi-object selection, global discretization, and beyond.
   %
   Extensive experiments demonstrate the effectiveness of our method on high-quality 3D segmentation and accurate hierarchical structure understanding.
   %
   A graphical user interface further facilitates flexible and real-time interaction for omniversal 3D segmentation. 
   %
   % The proposed method has the potential for advancing 3D scene understanding, which would further benefit downstream applications in the fields of robotics and virtual reality.\jinzhi{[Do we need this?]}
   % Code will be avaliable at XXX.



   % Towards holistic understanding of 3D scenes, a general 3D segmentation method is needed that can segment diverse objects without restrictions on object quantity or categories, while also reflecting the inherent hierarchical structure. To achieve this, we propose OmniSeg3D, an omniversal segmentation method aims for segmenting anything in 3D all at once. The key insight is to lift multi-view inconsistent 2D segmentations into a consistent 3D feature field through a hierarchical contrastive learning framework, which is accomplished by two steps. Firstly, we design a novel hierarchical representation based on category-agnostic 2D segmentations to model the multi-level relationship among pixels. 
   % Secondly, image features rendered from the 3D feature field are clustered at different levels of 2D segmentation blocks, which can be further drawn closer or pushed apart according to the hierarchical relationship between different levels. In tackling the challenges posed by inconsistent 2D segmentations, this framework yields a global consistent 3D feature field, which further enables hierarchical segmentation, multi-object selection, global discretization, and beyond. Extensive experiments demonstrate the effectiveness of our method on high-quality 3D segmentation and accurate hierarchical structure understanding. A graphical user interface further facilitates flexible and real-time interaction for omniversal 3D segmentation. 

   
\end{abstract}





% Towards holistic understanding of 3D scenes, there is a need for a general 3D segmentation method. This method should possess the capability to segment diverse objects without constraints on object quantity or categories, while also 
% %reflecting the 内在固有的 hierarchical structure of the 3D scene.
% incorporating a comprehension of the 3D scene structure.
% %
% To achieve this, we propose OmniSeg3D, an omniversal segmentation method aims for segmenting anything in 3D all at once. 
% %
% The basic idea is to lift 2D segmentations into 3D space, where the main challenge is to provide consistent 3D segmentations with inconsistent multi-view 2D masks. 
% %


% We first formulate a novel hierarchical representation for 2D observations with the help of category-agnostic 2D segmentation models. Then we design a contrastive learning strategy to distill the hierarchical knowledge from multi-view 2D images into 3D space, which results in a consistent 3D semantic feature field. This feature field further enables multi-object selection, hierarchical segmentation, as well as global discretization. 
% %
% Extensive experiments prove that our method enjoys high-quality 3D segmentation and has a correct understanding of hierarchical scene structure. 
% %
% A graphical user interface is also provided to realize flexible and real-time interaction for omniversal 3D segmentation. 
% %
% The proposed method has the potential for advancing 3D scene understanding at a higher level, which would benefit downstream applications in the fields of robotics and virtual reality.

==> sec/backup/1_intro_1031.tex <==
\section{Introduction}

% --- start from interaction --- %
% With the development of virtual reality, effective interaction with 3D world becomes a keen demand of people. The most basic form of interaction is object selection, which means people could choose 3D objects or part of them with simple click. This requires heavy work of art designers to design all the possible interactive contents. What we need is a method that support segment anything in 3D scenes all at once, which will enable more effective understanding and interaction in 3D scenes.

% --- start from holistic segmentation --- %

Humans are masters for 3D segmentation since they can tell apart anything in 3D world even without knowing the specific category or they have never seen the object before. Besides, it is easy for humans to understand the potential structure and function just by visual observation such as the relationship between objects and their parts.
%
% Inspired by the functionality of human visual system, an ideal 3D segmentation algorithm should have the ability to handle both common categories and unseen objects. Besides, it should have the ability to sense the hierarchical relationship between objects and parts. However the solution is nontrivial.
%
Inspired by the functionality of human visual system, an ideal 3D holistic segmentation algorithm should meets three requirements: \textbf{multiple objects} segmentation, \textbf{category-agnostic} segmentation,  \textbf{hierarchical} segmentation all at once in 3D. However the solution is nontrivial.

% The category-agnostic characteristic means the method should be able to handle unknown object categories and give instance segmentation of each object. 
% 
Standard 3D segmentation methods based on point cloud~\cite{han2020occuseg, liu2022insconv, kirillov2019panopticseg} and NeRF~\cite{zhi2021semanticnerf, siddiqui2023panopticlift, bhalgat2023contrastivelift} can segment multiple objects simultaneously. However, these methods can only handle pre-defined categories, which restricts the generalization ability and applications in open-world scenarios. 

With the emergence of powerful image models (like CLIP~\cite{radford2021clip}, LSeg~\cite{li2022lseg}, DINO~\cite{caron2021dino}), some methods propose to distill semantic-rich image feature onto point cloud~\cite{peng2023openscene, takmaz2023openmask3d} or NeRF~\cite{kerr2023lerf, kobayashi2022dff, goel2023isrf}. After distillation, users can segment objects with prompts (like point, scribble, and text) in a category-agnostic manner. However, due to the lack of boundary supervision, simply distilling these semantic feature into 3D space will lead to noisy segmentations~\cite{peng2023openscene, kerr2023lerf}. This can be relieved by finetuning the model with mask supervision~\cite{li2022lseg}, but this operation will weaken the open-vocabulary characteristic as well. So achieving both high segmentation quality and category-agnostic ability is difficult. Besides, multiple objects (instance) segmentation will be pretty hard for these methods since they rely on language-level or patch-level semantics. 
%
% In this paper we mainly focus on class-agnostic instance segmentation that can be applied in general scenes.

An effective way to achieve category-agnostic segmentation is ustilizing 2D segmentators like SAM~\cite{kirillov2023sam} or video segmentation methods~\cite{mirzaei2023spinnerf} to generate 2D mask of interested objects, and then lift them into 3D space~\cite{cen2023samin3d}. Though this kind of methods
% SAMin3D~\cite{cen2023samin3d} start from a segmentation of reference view and then propagates this mask to 3D space and other views via a pre-trained NeRF. SPInNeRF~\cite{mirzaei2023spinnerf} use a video segmentation method to get consistent masks and then optimize a consistent 3D mask for segmentation. 
have realized satisfactory results for single object segmentation, they can not segment multiple objects at once. 

For hierarchical segmentation, existing methods mainly focus on category-specific scenario~\cite{mo2019partnet, mo2019structurenet} or geometric analysis~\cite{chen2020bspnet, yu2022caprinet, yi2019gspn}, which are not suitable for general 3D scene segmentation. Therefore, realizing multi-object, category-agnostic, and hierarchical segmentation in 3D all at once is still an open question.

In this paper, we propose a method to achieve \textbf{Holistic 3D Segmentation via Hierarchical Contrastive Learning}. Our key idea is: category-agnostic 2D segmentations contains hierarchical information of objects and parts, which can be further integrated and aligned in 3D space via a hierarchical contrastive learning strategy. After that, the optimized feature field can be used to segment anything in 3D all at once. 

Specifically, we first construct a novel hierarchical representation for each 2D image with the help of click-based models. Click-based models like SAM provide a bunch of category-agnostic segmentation masks. By revisiting the relationship between these masks, we construct a patch-based representation and calculate hierarchical information between patches via a voting strategy.
%
Since the 2D hierarchical information may not be consistent across multi-view images, we design a contrastive learning framework to distill and align the multi-view hierarchical knowledge in 3D space, where the representation can be NeRF~\cite{mildenhall2021nerf} or Mesh. For each point in the 3D space, we define a continuous semantic feature as the instance identity. Then semantic features can be sampled, rendered to 2D, and supervised by patch-based contrastive regularization. Specifically, we identify the patch id for each rendered semantic feature. Then the feature distance between anchor patch and the other patches in different levels of the hierarchical tree are regularized by hierarchical loss weights and a forced optimization order.
%
After training, our method can directly give multi-view consistent semantic features, which enables multiple object selection, threshold-based scene hierarchy, as well as global discretization.

Our contributions are summarized as follows:
\begin{itemize}
    \item We propose a \textbf{hierarchical representation} to reveal and store the part-level relationship within objects based on class-agnostic 2D segmentation models and a voting strategy.
    \item We propose a \textbf{hierarchical contrastive learning method} to optimize a globally consistent 3D hierarchical feature field given 2D observations.
    \item Based on the hierarchical representation and contrastive learning method, we propose a \textbf{holistic 3D segmentation framework} to segment anything in 3D all at once, which enables flexible object selection, hierarchical thresholding, and 3D discretization.


\end{itemize}

==> sec/backup/1_intro_1101.tex <==
\section{Introduction}

% --- start from interaction --- %
% With the development of virtual reality, effective interaction with 3D world becomes a keen demand of people. The most basic form of interaction is object selection, which means people could choose 3D objects or part of them with simple click. This requires heavy work of art designers to design all the possible interactive contents. What we need is a method that support segment anything in 3D scenes all at once, which will enable more effective understanding and interaction in 3D scenes.

% --- start from holistic segmentation --- %

Humans are masters for 3D segmentation since they can tell apart anything in 3D world even without knowing the specific category or they have never seen the object before. Besides, it is easy for humans to understand the potential structure and function just by visual observation such as the relationship between objects and their parts.
%
% Inspired by the functionality of human visual system, an ideal 3D segmentation algorithm should have the ability to handle both common categories and unseen objects. Besides, it should have the ability to sense the hierarchical relationship between objects and parts. However the solution is nontrivial.
%
Inspired by the functionality of human visual system, an ideal 3D segmentation algorithm should also provide category-agnostic and hierarchical results. However the solution is nontrivial.


% Segmenting and interacting within 3D scenes has been a long standing and traditional subject in the field of computer vision for many years. This topic finds extensive use in areas such as virtual reality and the perception and visualization capabilities of robotics. 
% 
The category-agnostic characteristic means the method should be able to handle unknown object categories. 
% 
However, standard 3D segmentation methods like~\cite{han2020occuseg, liu2022insconv, kirillov2019panopticseg} can only handle pre-defined categories, which restricts the application in open-world scenarios.
Since there are not sufficient 3D datasets equivalent to massive 2D image datasets, a shortcut is to lift 2D segmentations into 3D space to realize 3D segmentation and inference.
%
With the emergence of powerful image models such as CLIP~\cite{radford2021clip}, LSeg~\cite{li2022lseg}, DINO~\cite{caron2021dino}, some methods propose to distill these image feature onto 3D representations such as point cloud~\cite{peng2023openscene, takmaz2023openmask3d} and NeRF~\cite{kerr2023lerf, kobayashi2022dff, goel2023isrf}. After distillation, user can interact with the 3D scenes with prompts such as point, scribble, and text. However, due to the lack of boundary supervision during training, simply distilling CLIP~\cite{radford2021clip} features into 3D space will cause noisy segmentations. This can be relieved by finetuning the model with mask supervision~\cite{li2022lseg}, but the open-vocabulary characteristic will be weakened as well. Besides, these methods may still be restricted by objects that can be described by language. In this paper we mainly focus on class-agnostic segmentation that can be applied in general scenes.


A more effective way is to use category-agnostic 2D segmentators like SAM~\cite{kirillov2023sam} to generate 2D mask of interested objects, and then lift them into 3D space~\cite{cen2023samin3d, mirzaei2023spinnerf}. SAMin3D~\cite{cen2023samin3d} start from a segmentation of reference view and then propagates this mask to 3D space and other views via a pre-trained NeRF. SPInNeRF~\cite{mirzaei2023spinnerf} use a video segmentation method to get consistent masks and then optimize a consistent 3D mask for segmentation. Though they have realized satisfactory results for single object segmentation, questions still lies in that how to segment every objects in a 3D scene all at once, i.e. holistic 3D segmentation.

In this paper, we propose a method to achieve \textbf{holistic 3D Segmentation via Hierarchical Contrastive Learning}. Our key idea is: category-agnostic 2D segmentations contains hierarchical information of objects and parts, which can be further integrated and aligned in 3D space via a hierarchical contrastive learning strategy, then the optimized feature field can be used to segment anything in 3D all at once. Specifically, we first construct a novel hierarchical representation for each 2D image. Click-based models like SAM provide a bunch of category-agnostic segmentations. By revisiting the relationship between these segmentations, we construct a patch-based representation and calculate hierarchical information between patches via a voting strategy.
%
Since the holistic 2D segmentations and the hierarchical information modeling may not be consistent across multi-view images, we design a contrastive learning framework to distill the multi-view hierarchical knowledge into 3D space via a consistent representation such as NeRF~\cite{mildenhall2021nerf} or Mesh. For each point in the 3D space, we define a continuous semantic feature as the instance identity. The semantic feature can be sampled and rendered to 2D feature for supervision. We apply patch-based contrastive regularization to optimize the semantic features on 2D images. Specifically, we identify the patch id for each sampled semantic feature. Then the feature distance between anchor patch and the other patches in different levels of the hierarchical tree are regularized by hierarchical loss weights and an ordered mask.
%
After training our method can directly give multi-view consistent semantic features, which enables click-based object choosing, threshold-based scene hierarchy, as well as global discretization.

The contributions of our method can be summarized as:
\begin{itemize}
    \item We propose a \textbf{hierarchical representation} to reveal and store the part-level relationship within objects based on class-agnostic 2D segmentation models and a voting strategy.
    \item We propose a \textbf{hierarchical contrastive learning framework} to optimize a globally consistent 3D hierarchical feature field given 2D observations.
    \item Based on the hierarchical representation and contrastive learning method, we propose a \textbf{holistic 3D segmentation framework} to segment anything in 3D all at once, which enables flexible object selection, hierarchical thresholding, and 3D discretization.


\end{itemize}
